Sliding Window Algorithms for k-Clustering Problems

The sliding window model of computation captures scenarios in which data is arriving continuously, but only the latest $w$ elements should be used for analysis. The goal is to design algorithms that update the solution efficiently with each arrival rather than recomputing it from scratch. In this work, we focus on $k$-clustering problems such as $k$-means and $k$-median. In this setting, we provide simple and practical algorithms that offer stronger performance guarantees than previous results. Empirically, we show that our methods store only a small fraction of the data, are orders of magnitude faster, and find solutions with costs only slightly higher than those returned by algorithms with access to the full dataset.

==> augment.tex <==
\paragraph{Augmented Meyerson Sketches} We now show how we can augment the sketch data structure with additional information for clustering in the sliding window model. \\
\emph{Maintaining Weights.} As we mentioned above, one of the challenges in adapting the Meyerson sketch to the sliding window setting lies in tracking the weight of a center as points expire. In fact, some of the points mapped initially to a center by $\mu$ may no longer be  part of the sliding window. Formally, given a stream $X = x_1, x_2, \ldots, x_t$, we would like to maintain an estimate of the weight of each center in $\centers$ restricted to the sliding window, i.e., for $\cen \in \centers$, we want to estimate $| \{ x \in W : \mu(x) = \cen\}|$. We denote this quantity by $\weight_\mu(\cen, X_{[t-w, t]})$. 
Maintaining an estimate of such a weight function falls directly into the Smooth Histograms framework introduced by \cite{Braverman07}. We leverage their approach to maintain a $(1 + \epsilon)$ estimate using only $\log _{1+\epsilon} w$ additional overhead per cluster center.
\begin{lemma}\label{lem:estimate-weight}
Fix constant $\epsilon>0$. Using additional space $O\left(|\centers| \log_{1+\epsilon}(w)\right)$, we can extend the Meyerson sketch $\centers, \weight$ with a function $\widehat{\weight} : \centers \times [n] \to \mathbb{Z}$ such that, at every time $t$, for every $ \cen \in \centers$, and every time $\tau$ in the active window: $\weight_\mu(\cen, X_{[\tau, t]}) \leq \widehat{\weight}(\cen,\tau) \leq (1+\epsilon) \weight_\mu(\cen, X_{[\tau, t]})$. 
\end{lemma}

\emph{Maintaining Centers.}
Our second task is making sure each cluster has a good center. Once again, this issue is unique to the sliding window setting, as in traditional data streams, points (and thus centers) never expire.  Specifically, whenever a center $\cen$ expires, we aim to replace it with a center $\cen'$ such that, $\dist(\cen, \cen')$ is small. In our context, small means comparable to the distance between the center $\cen$ and any point $x$ in the window that was mapped to it. 

\begin{definition}
Fix a mapping $\mu$ and a center $\cen$. We say that $y \in X_{[\tau, t]}$ is an $\epsilon$-replacement for $\cen$ at time $\tau$ if:
$\dist(\cen, y)^p \leq (1 + \epsilon) \dist(\cen, x)^p$ for any $x \in X_{[\tau, t]}$ with $\mu(x) = \cen$, where $t$ is the last time in the current stream.
\end{definition}

To obtain an $\epsilon$-replacement, we consider a sequence of concentric shells with geometrically increasing radii around each center $\cen$, and keep the last occurring point in every shell. Since distances are between $1$ and $\Delta$, we can bound the total number of shells by $O(\log_{1+\epsilon} \Delta)$ per center. When $\cen$ needs to be replaced, we simply look for the smallest non-empty shell and return its representative. By construction, we will ensure that the $\epsilon$-replacement property is satisfied. 


 \begin{lemma}\label{mapp:m}
Let $\epsilon \in (0,1)$, then with space $O(|\centers| \log_{1+\epsilon}(\Delta))$, it is possible to construct a function $\last : \centers \times [n] \to X$ that will always return an $\epsilon$-replacement for $\cen \in \centers$. 
\end{lemma}

\paragraph{Suffix Sketch}
The two augmentations before allow us to modify the Meyerson sketch in such a way that it can return an approximate solution 
for any suffix of the stream with length at most $w$. More precisely, we will show that we maintain a valid solution for the suffix 
with a cost comparable to the optimum of {\it the entire stream}.

\begin{lemma}\label{lemma:mb}
Let $w$ be the size of the sliding window, $\epsilon\in (0,1)$ be a constant and $t$ the current time. Let $(X,\dist)$ be a metric space and fix $ \gamma \in (0,1)$. The augmented Meyerson algorithm computes
an implicit mapping $\mu: X \rightarrow \centers$, and
 an $\epsilon$-consistent weighted instance $(\centers, \widehat{\weight})$ for all substreams $x_{[\tau, t]}$ with $\tau \geq t - w$ such that,  with probability $1- \gamma$, we have: 
$ |\centers| \leq 2^{2p+8} k \log  \gamma^{-1}\log \Delta \qquad {\text{and}} \qquad $
$ \cost_p(X_{[\tau,t]}, \centers)  \le  2^{2p+8} \opt_p(X).$\\
The algorithm uses space $O( k \log  \gamma^{-1} \log \Delta \log M/m (\log M + \log w + \log \Delta))$ and maintains the cost of the consistent mapping, $\cost(X, \mu)$, and also a $1+\epsilon$ approximation to the cost of the $\epsilon$-consistent mapping, $\widehat{\cost}(X_{[\tau, t]}, \mu)$.
\end{lemma}



==> meyerson-new.tex <==
\paragraph{Meyerson Sketches} We begin by formally stating the guarantees of the Meyerson sketch, giving a constant factor approximation for any constant $p$.\footnote{We do not optimize constants throughout the paper to keep proofs simpler. We empirically evaluate the algorithm's performance and show the efficacy of our approach.}
The following Lemma, captures the main properties of the sketch.

\begin{lemma}\label{lemma:corollary-of-lemma5o1}
Let $(X,\dist)$ be a metric space and fix $\gamma \in (0,1)$. Then the Meyerson sketch algorithm computes a mapping $\mu: X \rightarrow \centers$, and
a consistent weighted instance $(\centers$,$\weight$), such that $\centers \subseteq X$ and, with probability $1- \gamma$:
$
%$|C| \le 4k\log(\Delta)\log(\gamma^{-1})2^{2p+1}(1+\delta)^p$
|\centers| \leq 2^{2p+8} k \log  \nicefrac{1}{\gamma}\log \Delta {\text{;}} \quad 
\cost_p(X, \centers)  \le  2^{p+7} \opt_p(X).$
The algorithm uses at most  $2^{2p+8} k \log  \nicefrac{1}{\gamma}$ $\log \Delta \lceil\log M/m\rceil$ space and in the consistent mapping $\mu$, each point is mapped to a center inserted before it into the stream. 

\end{lemma}


